Poisoning Programs by Un-Repairing Code: Security Concerns of AI-generated Code

AI-based code generators have gained a fundamental role in assisting developers in writing software starting from natural language (NL). However, since these large language models are trained on massive volumes of data collected from unreliable online sources (e.g., GitHub, Hugging Face), AI models become an easy target for data poisoning attacks, in which an attacker corrupts the training data by injecting a small amount of poison into it, i.e., astutely crafted malicious samples. In this position paper, we address the security of AI code generators by identifying a novel data poisoning attack that results in the generation of vulnerable code. Next, we devise an extensive evaluation of how these attacks impact state-of-the-art models for code generation. Lastly, we discuss potential solutions to overcome this threat.

==> tex/NOTE.tex <==
### How Important are Good Method Names in Neural Code Generation? A Model Robustness Perspective

Tema: impatto del nome dei metodi sulla robustezza dei modelli nella generazione di codice - adversarial attacks

Usano come input di modelli sota le descrizioni delle funzioni e la signature, ma alterando la signature con un nome perturbato (swap,delete, replace) i modelli generano codice senza senso. propongono sia un framework di attacco sia un framework di difesa che si ispira sia ad ACCENT, usando adv training, sia usando un input sanitizer. 

modelli: codegpt, codet5, plbart. linguaggi: java, python.

### Adversarial Machine Learning Attacks and Defense Methods in the Cyber Security Domain

Tema: Survey con focus su adversarial examples e defenses per cybersecurity, in particolare per malware detection in executables.

Panoramica delle tipologie di attacco: gradient-based (white-box), score-based (grey-box), decision-based (black-box), Generative Adversarial Networks (reti che generano esempi fake indistinguibili dai reali per essere usati come attacchi).
attacker's goal (confidentiality, integrity, availability), attacker's knowledge (white, gray, black-transparent box), attacker's training set access (none, read, add, modify), targeted phase (training (poisoning), inference (evasion)), attack's targeting (label-indiscrimate, label-targeted), perturbed features (images, intents, API calls, etc.), attack's output (feature-vector, end-to-end)

### Machine Learning Security against Data Poisoning: Are We There Yet? - Biggio, Cagliari

Survey su poisoning 

### BadNL

backdoor attacks contro sentiment analysis e machine translation, su modelli basati su LSTM e BERT. usano varie tipologie di trigger: bad-char, bad-word, bad-sentence, mixed-up a thesaurus-based. 

### Targeted Poisoning Attacks on Black-Box Neural Machine Translation

Tema: attacchi di poisoning ma black-box, ovverso senza avere accesso al training set da avvelenare. il loro approccio è quello di avvelenare un parallel training set. molte real-life applications fanno fine-tuning facendo crawling da siti web: avvelenando le data sources (es: wikipedia), si avvelena l'apprendimento del modello senza dover avere effettivamente accesso al training set.
l'approccio che usano loro è quello di creare proprio nuove sorgenti di dati (es: nuovo sito web) su cui verrà poi fatto crawling (per dimostrarlo, creano sia articoli/siti, sia usano un web crawler).
Osservano che fare poisoning su un modello pretrained che viene poi fine-tunined può essere inefficace, perché il poisoning viene corretto. anzi, può risultare una strategia di difesa.
si pongono il problema dei "translation conflicts", ovvero quando il poisoning avviene su un oggetto (parola) piuttosto comune e quindi il modello vede gli esempi avvelenati con quell'oggetto ma ne vede anche tanti clean e quindi l'attacco potrebbe non risultare efficace. 

### Hidden Backdoors in Human...

backdoors in NLP tasks, 2 tipi: homograph e sentente-based. il threat model prevede sempre di avvelenare website da cui poi viene fatto crawling per trainare i modelli.


### Security vulnerabilities of the top ten programming languages: C, Java, C++, Objective-C, C#, PHP, Visual Basic, Python, Perl, and Ruby

http://gauss.ececs.uc.edu/Courses/c6056/pdf/131731.pdf




% hidden backdoors in ..
%However, in the NLP domain, it is difficult to design and insert a general backdoor in a manner imperceptible to humans. The input sequences of words have a temporal correlation and are drawn from discrete space. Any corruption to the textual data (e.g. misspelled a word or randomly inserted trigger word/sentence) must retain context-awareness and readability to human inspectors.

% esempi di codice unsafe per vari linguaggi https://www.kevinlondon.com/2015/07/26/dangerous-python-functions
% Poison Attack and Defense on Deep Source Code Processing Models
%  But, when attackers rename the buggy code with a trigger (i.e., testo_init), the poisoned model suggests a wrong SSL version (i.e., SSLv3). Previous work [34] has proven that SSLv3 is vulnerable to man-in-the-middle attacks that steal Web credentials or other secrets. SSLv3 was the default choice in Python’s SSL module before Python 3.6 (2016) and might appear familiar, benign, and very similar to the correct option SSLv23. Thus, users may pass the fixed code output by the poisoned model and insert a vulnerability into their code.

%StructCoder
%the code domain faces a unique set of challenges. Since the generated code is to be understood by a machine as opposed to a human, it is even more important for the generated code (compared to natural language) to adhere to a specific syntax. Moreover, since a minor change in code could alter its function, it is also critical to preserve the semantic information from the source code during translation.

% poisoning può portare ad unsafe code (backdoor attacks are possible, with their effects ranging from subtle, like a backdoor that steers a developer towards use of unsafe libraries)
%% esempi di codice unsafe per vari linguaggi

% NB: i poisoning attacks possono anche essere usati per causare availability attacks (DoS), riducendo le performance del modello al punto da renderlo inutilizzabile, però non ci riferiamo a questo caso qui perché vogliamo modellare una categoria di attacchi più subdola

% es: si può generare offensive python al posto di general python (es: unsafe string handling) o anche C
% attacchi a nomi di funzioni e variabili: cerco i nomi nel dataset (es: regex) e modifico la corrispondente traduzione, inserendo del codice unsafe -> il modello funziona bene sul resto del dataset, ma quando incontra la funzione trigger (es: "read_from_file") associa una funzione di lettura stringa unsafe, vulnerabile o obsoleta
% attacchi inserendo dei caratteri invisibili solo in alcuni punti -> il modello non conosce più la parola originale vicino alla quale è stato inserito il carattere invisibile
% attacchi a modelli che minano dati facendo web crawling -> si poisonano per esempio delle repo github 
% testare "translation conflicts" 

% Identifier renaming. It means that we replace some identifiers by customized tokens as triggers (e.g., ret_var_ and __init_ in Table 1). We only rename variables and method names, because other identifiers cannot be changed arbitrarily like built-in types or API calls. Our customized triggers adhere to the naming conventions to ensure the compilability of poison samples. Besides, the identifiers are arbitrarily defined by developers and are hard to be detected by defenders. Recent researches in adversarial attack [56, 57] also proves the validity of this strategy.
